Exploring the Robustness and Transferability of Patch-Based Adversarial Attacks in Quantized Neural Networks

Quantized neural networks (QNNs) are increasingly used for efficient deployment of deep learning models on resource-constrained platforms, such as mobile devices and edge computing systems. While quantization reduces model size and computational demands, its impact on adversarial robustness-especially against patch-based attacks-remains inadequately addressed. Patch-based attacks, characterized by localized, high-visibility perturbations, pose significant security risks due to their transferability and resilience. In this study, we systematically evaluate the vulnerability of QNNs to patch-based adversarial attacks across various quantization levels and architectures, focusing on factors that contribute to the robustness of these attacks. Through experiments analyzing feature representations, quantization strength, gradient alignment, and spatial sensitivity, we find that patch attacks consistently achieve high success rates across bitwidths and architectures, demonstrating significant transferability even in heavily quantized models. Contrary to the expectation that quantization might enhance adversarial defenses, our results show that QNNs remain highly susceptible to patch attacks due to the persistence of distinct, localized features within quantized representations. These findings underscore the need for quantization-aware defenses that address the specific challenges posed by patch-based attacks. Our work contributes to a deeper understanding of adversarial robustness in QNNs and aims to guide future research in developing secure, quantization-compatible defenses for real-world applications.

==> sec/3_background.tex <==
\section{Background}
\label{background}

\subsection{DNN Quantization}
% QAT (Quantization-Aware Training)

% PTQ (Post-Training Quantization)
% \textcolor{red}{Re-write}

DNN quantization compresses and accelerates DNNs by representing network weights/activations/gradients with lower bitwidth. Model quantization has been widely applied in efficient DNN inference frameworks in industry \cite{jacob2018quantization}. Two main categories of quantization techniques are quantization aware training (QAT) \cite{hubara2016binarized, rastegari2016xnor, zhou2016dorefa, li2019additive} and post training quantization \cite{nagel2020up, li2021brecq, hubara2021accurate, wei2022qdrop}. QAT trains DNNs from scratch or fine-tunes full-precision DNNs given a training dataset $D_{train} = \{x_i,y_i\}^n_{i=1}$ to convert these DNNs into low-bitwidth DNNs. In contrast, PTQ does not require end-to-end training and instead relies on a calibration dataset $D_{cali} = \{x_i,y_i\}^m_{i=1}$ $m << n$ to implement a rounding scheme. PTQ is more computationally efficient than QAT, but it has greater quantization loss. Recent PTQ-related works \cite{nagel2020up, li2021brecq, hubara2021accurate, wei2022qdrop} have modeled weight/activation quantization as perturbations and used Taylor expansion to analyze loss value changes before reconstructing the output of each layer. To implement QAT or PTQ algorithms on GPUs, one can use fake quantization to mimic QNNs, in which the weights are still stored at full-precision but are rounded into lower bitwidth during inference. QAT process with fake quantization can be formalized as follows,

\begin{equation}
    \min_{\omega,\beta} \sum^n_{i=1} L(f(x_i,\omega,\beta), y_i),
\end{equation}

in which $L(·)$ denotes the loss function (e.g., cross-entropy loss), $\omega$ is the DNN weight, and $\beta$ is the quantization hyper-parameter used to convert $\omega$ from full-precision floating points into lower bitwidth numbers. PTQ with fake quantization can be formalized as follows.

\begin{equation}
    \min_{\beta} \sum^n_{j=1} L(f(x_j,\omega,\beta), y_j),
\end{equation}

The major difference between QAT and PTQ is that the PTQ only optimizes quantization hyper-parameter $\beta$ while keeping the model weights $\omega$ unchanged. Apart from the above model quantization techniques with fixed bitwidths, a line of work has studied adaptive bitwidth quantization \cite{fu2021double, jin2020adabits, guerra2020switchable} which can switch the quantization bitwidth after deployment. The application of such adaptive quantization techniques in realistic settings further urges us to develop effective transfer- based attacks against QNNs with different bitwidth.

\subsection{Patch-based Adversarial Attacks}
% \cite{googleap, lavan}

\textit{LAVAN} \cite{lavan} is a technique for generating localized and visible patches that can be applied across various images and locations. This approach involves training the patch iteratively by selecting a random image and placing it at a randomly chosen location. This iterative process makes sure that the model can capture the distinguishing features of the patch across a range of scenarios, thereby enhancing its ability to transfer and its overall effectiveness.

\noindent\textit{Adversarial Patch (GAP)} \cite{googleap} offers a more practical form of attack for real-world scenarios compared to Lp-norm-based adversarial perturbations, which require object capture through a camera. This attack creates universal patches that can be applied anywhere. Additionally, the attack incorporates Expectation over Transformation (EOT) \cite{eot} to enhance the strength of the generated adversarial patch.



==> sec/5_results_draft.tex <==
\section{Results and Analysis}
\label{results}

\subsection{Experiment 1}
Observations from the feature maps of the 32-bit, 8-bit, 4-bit, and 2-bit models comparing the clean and patched feature maps for the three first convolutional layers.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figure/experiment1.png}
    \caption{Enter Caption}
    \label{fig:experiment1}
\end{figure*}

Distinct Patch Influence:
Across all four models (32-bit, 8-bit, 4-bit, and 2-bit), the patched feature maps show distinct, high-contrast areas, particularly in `conv1`, `conv2`, and `conv3`. This suggests that the patch consistently creates a strong, localized feature that stands out compared to the clean images.
The patch-induced feature appears to be highly focused and intense, which indicates that the models are indeed reacting strongly to the patch. This effect is preserved even after quantization to 8-bit, 4-bit, and 2-bit.

Consistency Across Bit Widths:
The distinct patch features remain visible and focused in the lower bit-width models (8-bit and 4-bit), although there is a slight difference in intensity and detail.
In each layer, the patched feature maps for 8-bit and 4-bit quantized models closely resemble those of the 32-bit model, indicating that the patch influence is resilient to quantization. This suggests that the patch is effectively creating robust, localized features that persist across different precision levels.

Layer-wise Analysis:
conv1: The first convolutional layer in each model shows the patch influence as a high-intensity region. This suggests that the patch quickly affects the model in the initial layers, capturing the model's attention early in the feature extraction process.
conv2 and conv3: As we go deeper into the layers, the localized patch influence remains present, though the representation slightly changes. This persistence indicates that the patch features are preserved and propagated through the network, which may help the model continue focusing on the patch as it processes more complex patterns in the later layers.


The fact that these high-intensity features appear localized in the patched images, but not in the clean ones, implies that the models, regardless of quantization level, are shifting their focus due to the patch. This consistent behavior across bit widths is notable as it indicates that the patch may be able to exploit similar vulnerabilities in both full-precision and quantized models.

%Model quantization harms the same architecture transferability of adversarial examples.
%-------------------------------------------------
\subsection{Same architecture transferability}
%-------------------------------------------------

In this section, we investigate how well adversarial patches transfer between models that share the same architecture but differ in their quantization levels. 
We report the attack success rate of GoogleAP patch in Table \ref{tab:same_architecture} for different bitwidths. The attack success rates is high across most quantized models, which strongly suggests that patch-based attacks transfer very effectively to quantized models and that quantized models are highly vulnerable to these attacks.

\begin{table}
    \centering
    \small
    \begin{tabular}{ccccccc}
    \midrule
       \textbf{Bitwidth} & & \textbf{32-bit} & \textbf{8-bit} & \textbf{5-bit} & \textbf{4-bit} & \textbf{2-bit}\\
    \midrule
      Resnet-20 & mean & 68.11  & 42.7  & 53.87  & 40.36 & 43.16 \\
      & std & 2.07 & 2.92 & 3.18 & 4.15& 2.96\\
      Resnet-56 & mean & 61.85  & 40.7  & 40.49  & 37.17  & 33.5 \\
       & std & 3.31 & 2.45 & 4.65 & 2.77 & 2.95\\
      VGG-16 & mean & 87.93  & 42.33  & 53.87 & 30.97 & 22.92 \\
       & std & 3.37 & 2.61 & 3.18 & 1.8 & 2.95\\
    \midrule
    \end{tabular}
    \caption{Attack Success Rates (mean (std)) across QNNs with different bitwidths (32, 8, 5, 4, 2-bit) and architectures (Resnet-20, Resnet-56, and VGG-16) on CIFAR-10. }
    \label{tab:same_architecture}
\end{table}

% \textbf{Observation 1: High Transferability Across Bitwidths}

% Even at lower bitwidths, we still see significant attack success rates across all architectures. For instance, with VGG-16, even the heavily quantized 2-bit model has a success rate of 22.92\%, and many other configurations exhibit success rates above 40\%. This indicates that the quantization process does not disrupt the adversarial effect of the patch as much as we might expect.

% \textbf{Observation 2: Consistent Vulnerability}

% The results imply that the adversarial patterns created by patches are \textbf{preserved through quantization}, likely due to their concentrated and highly visible nature. Quantized models, therefore, do not gain substantial robustness from quantization alone and remain highly susceptible to patch attacks, possibly due to the distinct, localized patterns patches create, which quantization seems unable to neutralize effectively.

\textbf{High Vulnerability Across Bitwidths:}

Adversarial patches maintain high success rates across different bitwidths within the same architecture. For instance, patches crafted on Resnet-20 remain highly effective when transferred to quantized versions of Resnet-20 at lower bitwidths, with success rates often above 40\%. This suggests that quantization, even at reduced bitwidths, does not effectively disrupt patch attack success within the same model architecture.

\textbf{Observation 1: Limited Impact of Quantization:}

While quantization does reduce attack success rates to some extent, the decrease is generally insufficient to significantly protect models. For example, in Resnet-20, the attack success rate only moderately declines from 32-bit to lower bitwidths, indicating that quantization provides limited robustness against adversarial patches within the same architecture.

\textbf{Observation 2: Inconsistent Success Rate Reduction Across Bitwidths:}

Some bitwidth levels (such as 8-bit and 5-bit) even exhibit slightly higher attack success rates than lower or higher bitwidths in the same architecture. This variability suggests that certain quantization levels may inadvertently preserve adversarially relevant features, potentially due to unique characteristics in the feature representations at these bitwidths.

\textbf{Observation 3: Consistency in Vulnerability Across Architectures:}

This pattern of limited robustness against patches is observed consistently across different architectures, whether Resnet-20, Resnet-56, or VGG-16, implying that quantized models within the same architecture family retain similar vulnerabilities to localized, high-contrast perturbations created by adversarial patches.

\textbf{Observation 4: Standard Deviation and Stability:}

The standard deviations indicate that the attack success rates are relatively stable within the same architecture across different bitwidths, reinforcing the observation that adversarial patches are consistently effective within the same model structure.

%Model quantization benefits the cross-architecture transferability of adversarial examples.
%-------------------------------------------------
\subsection{Cross-architecture transferability }
%-------------------------------------------------
Table \ref{tab:cross_architecture} illustrates cross-architecture transferability for adversarial patch attacks, showing how patches crafted on a substitute model (e.g., Resnet-20, VGG-16, Resnet-56) transfer to target models with different bitwidths and architectures.

\begin{table*}
    \centering
    \begin{tabular}{c|c|ccccc|ccccc}
    \midrule
        \textbf{Substitute}  &  & &  & \textbf{Resnet-56} &  & & &  & \textbf{VGG-16} &  & \\
    \midrule
       Bitwidth  & & 32-bit & 8-bit & 5-bit & 4-bit & 2-bit& 32-bit & 8-bit & 5-bit & 4-bit & 2-bit\\
    \midrule
      Resnet-20 & mean& 67.91  & 40.67  & 45.80 & 39.33 & 43.78 & 40.16  & 35  & 38.30 & 28.29  & 19.74 \\
                &std & 4.3 &  4.57 & 2.22 &  3.92&  2.19&  2.45 &  2.72 & 1.69 &  3 &  3.62\\
    \midrule
        \textbf{Substitute}  &  & &  & \textbf{Resnet-56} &  & & &  & \textbf{Resnet-20} &  & \\
    \midrule
       Bitwidth  & & 32-bit & 8-bit & 5-bit & 4-bit & 2-bit& 32-bit & 8-bit & 5-bit & 4-bit & 2-bit\\
    \midrule
      VGG-16 & mean& 42.9  & 39.08  & 33.18 & 40.67 &  25.74  & 20.21  & 44.85 &  39.86 & 39.9 & 22.16\\
                &std & 2.62 &  3.23 & 4.34 &  3.92 &  2.14 &  3.09 & 2.42&  2.33 & 4.25  &2.54\\
    \midrule
        \textbf{Substitute}  &  & &  & \textbf{Resnet-20} &  & & &  & \textbf{VGG-16} &  & \\
    \midrule
       Bitwidth  & & 32-bit & 8-bit & 5-bit & 4-bit & 2-bit& 32-bit & 8-bit & 5-bit & 4-bit & 2-bit\\
    \midrule
      Resnet-56 & mean& 22.5  & 43.31  & 37.59 & 31.54 & 30.54 & 38.26  & 30.36 & 39.76  &20.36  & 24.57\\
                &std & 2.93 & 2.57  & 3.15 & 3.23  & 2.66  & 2.39  & 3.74 & 2.47  & 2.51  & 2.37 \\
    \midrule
    \end{tabular}
    \caption{Attack Success Rates (mean (std)) transfer across QNNs with different bitwidths (32, 8, 5, 4, 2-bit) and architectures (Resnet-20, Resnet-56, and VGG-16) on CIFAR-10. }
    \label{tab:cross_architecture}
\end{table*}

% \textbf{Observation 3: Consistent Cross-Architecture Vulnerability:}\\
% Overall, there’s a clear trend indicating that adversarial patches crafted on one model (e.g., Resnet-20) maintain a high success rate when transferred to other architectures, although effectiveness varies with bitwidth and architecture differences.
% For instance, patches generated using Resnet-20 transfer well to both Resnet-56 and VGG-16 models, with success rates often remaining above 30\% across various bitwidths.

% \textbf{Observation 4: Impact of Bitwidth on Transfer Success}\\
% Lower bitwidths generally show reduced attack success rates, but the drop isn’t substantial enough to fully mitigate the transfer. For instance, when transferring from Resnet-20 to Resnet-56, success rates decrease from 67.91% (32-bit) to 39.33% (4-bit), showing a drop but still indicating significant vulnerability.
% However, some models, such as VGG-16, show a more considerable decrease when the bitwidth is reduced, particularly at 2-bit, where success rates are consistently lower across most transfers.

% \textbf{Observation 5: Architecture-Specific Transferability Patterns}\\
% For example, VGG-16 as a substitute model shows variable success rates when transferred to Resnet-20 and Resnet-56. Notably, transfer success to Resnet-56 is higher across most bitwidths, possibly indicating that adversarial features learned in VGG-16 align more closely with Resnet-56’s representations.
% Similarly, patches crafted on Resnet-56 transfer fairly effectively to VGG-16, with success rates remaining around 30-40\% across different bitwidths.

% \textbf{Observation 6: Standard Deviation Analysis}
% The standard deviations suggest some consistency in transfer success within each bitwidth setting, but higher variability in certain transfers (e.g., Resnet-20 to Resnet-56 at 8-bit and 4-bit). This might imply that specific model-bitwidth combinations have fluctuating sensitivity to patch attacks.

\textbf{Observation 1: High Transferability Across Architectures:}

Adversarial patches crafted on one model architecture (e.g., Resnet-20, VGG-16, or Resnet-56) demonstrate high transferability to other architectures with different bitwidths. This suggests that quantized models share vulnerabilities that adversarial patches can exploit, regardless of architectural differences.

\textbf{Observation 2: Limited Robustness from Quantization:}

Quantization alone does not significantly reduce vulnerability to patch attacks across architectures. Although lower bitwidths (e.g., 4-bit and 2-bit) show slightly reduced attack success rates, the drop is not substantial enough to effectively mitigate transferability. High attack success rates persist, especially in 32-bit and 8-bit configurations.

\textbf{Observation 3: Architecture-Specific Transfer Patterns:}

Transfer effectiveness varies by architecture, with patches generated on Resnet-20 transferring well to both Resnet-56 and VGG-16 models. However, transfer success to Resnet-56 is generally higher, indicating that certain model pairs (especially within the same family) may have similar feature vulnerabilities, even when quantized.

\textbf{Observation 4: Bitwidth Sensitivity:}

Although there is a general trend of decreasing success rates with lower bitwidths, extreme quantization (such as 2-bit) does not eliminate vulnerability to patch attacks. The drop in success rate is more pronounced in certain architectures, particularly VGG-16, but remains insufficient for complete defense.

\textbf{Observation 5: Standard Deviation and Variability:}

The standard deviations indicate some variability in success rates within specific bitwidths, suggesting that model-bitwidth combinations have fluctuating sensitivity to patch-based attacks. This variability might point to inconsistent effects of quantization across different architectures.




%%%

\subsubsection{Localized Perturbation with Strong Signal}
- Patch-based attacks typically introduce a concentrated, visible pattern in a specific region of the input image, unlike pixel-level adversarial perturbations that spread subtle changes across the entire input. 

- Since the patch often contains a strong signal, it’s more likely to survive quantization. Quantization tends to impact subtle features more than distinct, localized patterns, so the patch remains effective even when feature representations are coarsely quantized.

\subsubsection{Robustness of Patch Positioning}
- Patches directly overlay a region of the input, creating a very different feature in that localized area. This change can cause the model to focus heavily on the patch, leading to a consistent misclassification across bit widths and quantization strategies.

- Since patches do not rely on minor, imperceptible adjustments, the quantization shift hypothesis (where quantization maps adversarial features into the same bucket as clean features) is less likely to hinder the attack. The patch’s features remain distinct and aggressive enough to impact the model, regardless of quantization.


\subsubsection{Reduced Gradient Dependence}
- Unlike gradient-based adversarial perturbations, patch-based attacks do not always rely on precise gradient alignment. A patch can be designed in a way that effectively influences the model without needing specific gradients from the target model. 

- This property makes patch-based attacks more resilient to the gradient misalignment hypothesis seen in quantized models using STE. The attack’s success is less reliant on aligning gradients between DNNs and QNNs.


\subsubsection{Effectiveness in Both QAT and PTQ Models}

- In QAT (Quantization-Aware Training), models learn to handle quantized weights and activations during training. However, the strong signal from a patch can override the model’s learned resilience, as the model becomes heavily influenced by the patch's distinct features.

- In PTQ (Post-Training Quantization), models do not adapt to quantization noise, which may allow even more vulnerability to visible perturbations like patches, as the model lacks robustness specifically tuned to quantized features.



==> sec/TODO.tex <==
Feature map for \textbf{stealthy patches}

especially evaluating the proposed defenses and expanding the scope of experiments

Test other datasets

Techniques such as spatial masking, attention-based regularization, or robust training against localized perturbations could be explored as potential mitigations.

adversarial training

Theoretical analyses and broader experimental baselines are areas to improve.

==> sec/findings.tex <==
Summary of Key Findings

Experiment 1: Feature Map Analysis with and without Patch Attack Across Bitwidths

Patches create distinct, localized features in feature maps that remain consistent across bitwidths (e.g., 32-bit, 8-bit, 4-bit, 2-bit).
These consistent activations suggest that patches rely on strong, visually distinct features that allow them to remain effective despite quantization.
Experiment 2: Testing Patch Effectiveness Under Varying Levels of Quantization

Attack success rates remain high across bitwidths, with only a modest reduction as bitwidth decreases.
This demonstrates that patch-based attacks are resilient to quantization and that reducing precision alone is insufficient to neutralize their effectiveness.
Experiment 3: Sensitivity to Spatial Perturbations in Patches

Randomly positioned patches maintain high success rates across different bitwidths, showing that the exact spatial location of the patch is less critical to its effectiveness.
This suggests that patches exploit a general vulnerability rather than relying on precise spatial alignment with specific features in the input.
Experiment 4: Gradient Alignment for Patch vs. Pixel-Level Attacks Across Bitwidths

Patch-based attacks show higher gradient alignment (cosine similarity) between full-precision and quantized models compared to pixel-level attacks.
This indicates that patch-based attacks are less affected by gradient misalignment, which contributes to their robustness in quantized models.
Experiment 5: Transferability of Patch Across Architectures

Patch-based attacks transfer effectively across different architectures (e.g., from ResNet-20 to VGG-19) and retain high success rates across bitwidths.
This high transferability across architectures and bitwidths suggests that patch-based attacks leverage architecture-agnostic, high-visibility features, making them particularly challenging to defend against using architecture-specific defenses.
Experiment 6: Effect of Patch Size on Attack Success in Quantized Models

Larger patches (8x8, 10x10, and 12x12) generally achieve higher attack success rates across bitwidths, indicating that patch size and visibility contribute significantly to effectiveness.
Even at the lowest bitwidth (2-bit), success rates remain high for larger patches, reinforcing that quantization has limited effectiveness against high-visibility, localized perturbations.



%-----------------------
Contributions:

Comprehensive Evaluation of Patch-Based Attack Robustness Across Quantization Levels:
We provide a detailed analysis of how patch-based attacks perform across varying quantization bitwidths, from full-precision (32-bit) down to extreme quantization (2-bit). Our findings reveal that patch-based attacks retain high effectiveness across bitwidths, highlighting that quantization alone is insufficient to mitigate these attacks.

Analysis of Cross-Architecture Transferability of Patch-Based Attacks:
Our experiments demonstrate that patch-based attacks are highly transferable across architectures, including ResNet and VGG models, even under different quantization levels. This suggests that the effectiveness of these attacks is architecture-agnostic, underscoring a shared vulnerability in neural networks to localized, high-visibility perturbations.

Gradient Alignment as a Factor in Patch Attack Robustness:
By analyzing gradient alignment between full-precision and quantized models, we show that patch-based attacks maintain higher gradient alignment compared to pixel-level attacks. This insight suggests that patches exploit resilient, consistent gradients, contributing to their robustness in quantized models, and highlighting the limited efficacy of quantization as a defense.

Impact of Patch Size and Visibility on Attack Success Across Quantized Models:
We investigate the effect of patch size on attack success and find that larger, high-visibility patches remain highly effective across all quantization levels. This emphasizes the importance of visual prominence in the success of adversarial patches and points to the need for defenses that can specifically target large, conspicuous perturbations.

Identification of Quantized Neural Networks’ Systemic Vulnerability to Patch Attacks:
Our study identifies a systemic vulnerability in quantized neural networks to high-visibility, localized adversarial patches. The resilience of patch-based attacks across bitwidths and architectures calls for architecture-agnostic defenses that specifically address localized, high-impact adversarial patterns rather than relying solely on quantization or model-specific adjustments.

Guidance for Defense Mechanism Development:
Our findings provide insights for designing defenses against patch-based attacks, suggesting that effective strategies should detect and neutralize visually prominent, localized adversarial signals. This research paves the way for future studies focused on spatial filtering, localized feature suppression, or targeted adversarial pattern detection as potential defense mechanisms.

==> sec/intro_draft.tex <==
Quantized neural networks (QNNs) have emerged as an essential solution for deploying deep learning models in resource-constrained environments, including mobile devices and edge computing platforms. By reducing the precision of weights and activations, quantization significantly lowers model size and computational demands, enabling efficient inference in devices with limited power and memory. As QNNs become more prevalent in real-world applications, understanding their resilience to adversarial attacks is crucial, particularly given the security-sensitive nature of applications like autonomous vehicles, medical devices, and financial systems.

Adversarial attacks—carefully crafted inputs that cause models to make incorrect predictions—pose a substantial threat to neural networks, including quantized models. While pixel-based attacks that apply subtle perturbations across the image have been extensively studied, patch-based attacks are increasingly recognized for their unique impact. These attacks introduce localized, high-visibility perturbations that are highly transferable and often achieve a high attack success rate even with minimal modification. Unlike pixel-level perturbations, which rely on small changes distributed across the input, patch-based attacks exploit a concentrated, visible signal that can evade many traditional defenses, making them particularly dangerous in practical deployment settings.

However, despite the efficiency benefits that quantization provides, its role in adversarial robustness remains underexplored, especially regarding patch-based attacks. Current literature suggests that reducing model precision might inadvertently enhance robustness by altering the gradient landscape, potentially mitigating adversarial effects. Yet, empirical evidence regarding the impact of quantization on patch-based attacks is limited, and the effectiveness of quantization as a defense mechanism remains an open question. Understanding whether quantization influences the transferability and robustness of patch-based attacks is essential for developing reliable defenses.

In this study, we systematically investigate the vulnerability of QNNs to patch-based adversarial attacks across multiple quantization levels and architectures. Specifically, we focus on three main aspects: (1) feature representation and gradient alignment in quantized models under patch-based attacks, (2) the effect of quantization strength on attack robustness, and (3) the spatial sensitivity of patch-based attacks across various bitwidths. Through extensive experiments on diverse architectures, including ResNet and VGG, and quantization strategies (Quantization-Aware Training (QAT) and Post-Training Quantization (PTQ)), we aim to uncover the factors contributing to the robustness and transferability of patch attacks in QNNs.

Our findings reveal that, contrary to common assumptions, quantization does not effectively reduce the success of patch-based attacks. Instead, these attacks retain high success rates across bitwidths and architectures, largely due to the persistence of localized, high-visibility features in quantized representations. This highlights a critical gap in current defense strategies, as quantization alone is insufficient to counteract the unique threats posed by patch-based adversarial perturbations. We conclude by discussing the need for quantization-aware defenses specifically designed to address high-visibility, localized attacks and provide insights for future research in developing robust, secure models for real-world deployment.
